Mixture of segmentation for heterogeneous functional data

In this paper we consider functional data with heterogeneity in time and in population. We propose a mixture model with segmentation of time to represent this heterogeneity while keeping the functional structure. Maximum likelihood estimator is considered, proved to be identifiable and consistent. In practice, an EM algorithm is used, combined with dynamic programming for the maximization step, to approximate the maximum likelihood estimator. The method is illustrated on a simulated dataset, and used on a real dataset of electricity consumption.

==> Fig/Transformation_data_real_VB.tex <==
%%%% Curve
\draw[domain=0.1:5.6, samples=112] plot (\x, {-sin(\x/2.4*2*pi r)/2+cos(\x*7*pi r)/6-cos(\x*11*pi r)/10}) ;
\draw[domain=5.6:5.75, samples=6,dotted] plot (\x, {-sin(\x/2.4*2*pi r)/2+cos(\x*7*pi r)/6-cos(\x*11*pi r)/10}) ;
\draw[dotted] (6.575,0) -- (7.575,0);
\draw[domain=5.4:5.6, samples=5,dotted] plot (\x+3, {-sin((\x-12.8)/2.4*2*pi r)/2+cos((\x-12.8)*7*pi r)/6-cos((\x-12.8)*11*pi r)/10}) ;
\draw[domain=5.6:8, samples=49] plot (\x+3, {-sin((\x-12.8)/2.4*2*pi r)/2+cos((\x-12.8)*7*pi r)/6-cos((\x-12.8)*11*pi r)/10}) ;
%%% Scale
%% Begin
\foreach \t in {0.05,0.1,...,5.8}
    {\draw[opacity=0.5] (\t,-1.05) -- (\t,-0.95);}
\foreach \d in {0,2.4}{
    \foreach \t in {4,8,...,24}
        {\draw[opacity=0.75] (\t/10+\d,-1.05) node[below]{\tiny{\t}};}
        }
\foreach \t in {4,8}
    {\draw[opacity=0.75] (\t/10+4.8,-1.05) node[below]{\tiny{\t}};}
%% End
\foreach \t in {5.5,5.55,...,8.05}
    {\draw[opacity=0.5] (\t+3,-1.05) -- (\t+3,-0.95);}
\foreach \t in {4,8,12,16,20,24}
    {\draw[opacity=0.75] (\t/10+8.6,-1.05) node[below]{\tiny{\t}};}
\foreach \t in {24}
    {\draw[opacity=0.75] (\t/10+6.2,-1.05) node[below]{\tiny{\t}};}
%% Days
\foreach \x in {0,2.4,4.8,8.6,11}{
    \draw[red,dashed,opacity=0.5] (\x,-1) -- (\x,1);}
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (0,-1.5) -- (2.4,-1.5) node [midway,below=8pt] {\tiny January 1st, 2020};
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (2.4,-1.5) -- (4.8,-1.5) node [midway,below=8pt] {\tiny January 2nd, 2020};
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (4.8,-1.5) -- (7.2,-1.5);
\fill[white] (5.6,-1.5) rectangle (8.6,-2);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (4.8,-1.5) -- (7.2,-1.5);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (6.2,-1.5) -- (8.6,-1.5);
\fill[white] (5.75,-1.5) rectangle (8.4,-2);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (8.6,-1.5) -- (11,-1.5) node [midway,below=8pt] {\tiny December 31st, 2020};
%% Arrow
\draw[opacity=0.5] (0,-1) -- (5.9,-1);
\draw[opacity=0.5,dotted] (8.35,-1) -- (6,-1);
%\draw[opacity=0.5,dotted] (8.5,-1) -- (6.25,-1);
\draw[->,>=latex,opacity=0.5] (8.35,-1) -- (11.5,-1);
%%%%%%%%%%%%%
% Case
%%%%%%%%%%%%%
%%% Day, week
% Day
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (0,-4) -- (5,-4) node [midway,below=8pt] {\tiny January 1st, 2020};
\fill[white] (3.2,-4) rectangle (3.8,-4.25);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (0,-4) -- (5,-4);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (5,-4) -- (8,-4);
\fill[white] (6,-4) rectangle (7,-4.5);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (5,-4) -- (8,-4);
\fill[white] (6.2,-4) rectangle (6.8,-4.5);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror}] (8,-4) -- (11,-4);
\fill[white] (9,-4) rectangle (9.9,-4.5);
\draw[red,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (8,-4) -- (11,-4);
\fill[white] (9.2,-4) rectangle (9.7,-4.5);
% Week
\draw[blue,decorate,decoration={brace,amplitude=10pt,mirror}] (0,-4.5) -- (8,-4.5) node [midway,below=8pt] {\tiny First Week};
\fill[white] (3.2,-4.5) rectangle (3.8,-4.75);
\fill[white] (6,-4.5) rectangle (7,-4.75);
\draw[blue,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (0,-4.5) -- (8,-4.5);
% end
\draw[blue,decorate,decoration={brace,amplitude=10pt,mirror}] (8,-4.5) -- (11,-4.5);
\fill[white] (9,-4.5) rectangle (9.9,-4.75);
\draw[blue,decorate,decoration={brace,amplitude=10pt,mirror},dotted] (8,-4.5) -- (11,-4.5);
\fill[white] (9.2,-4.5) rectangle (9.7,-5);
%%% Begin
\draw (0,-3.5) grid[ystep=0.5,xstep=1] (3.2,-4);
\foreach \h in {1,2,3}{
    \draw (\h-0.5,-3.75) node{\tiny$X_{i\h}(t_{\textcolor{blue}{1}})$};
    }
%%% End first day
\draw (3.5,-3.75) node{$\cdots$};
\draw (3.8,-3.5) grid[ystep=0.5,xstep=1] (6.2,-4);
\draw (4.5,-3.75) node{\tiny$X_{i24}(t_{\textcolor{blue}{1}})$};
\draw (5.5,-3.75) node{\tiny$X_{i25}(t_{\textcolor{blue}{1}})$};
%%% End first week
\draw (6.5,-3.75) node{$\cdots$};
\draw (6.8,-3.5) grid[ystep=0.5,xstep=1] (9.2,-4);
\draw (7.5,-3.75) node{\tiny$X_{i336}(t_{\textcolor{blue}{1}})$};
\draw (8.5,-3.75) node{\tiny$X_{i1}(t_{\textcolor{blue}{2}})$};
%%% End 
\draw (9.45,-3.75) node{$\cdots$};
\draw (9.7,-3.5) grid[ystep=0.5,xstep=1.1] (11,-4);
\draw (10.45,-3.75) node{\tiny$X_{i336}(t_{\textcolor{blue}{52}})$};
%%%%%%%%%%%%%%%%%%%%%
% Transformation
%%%%%%%%%%%%%%%%%%%%%
%% Grid
% Haut
\draw (2,-7) grid (5.2,-9.2);
\draw (5.8,-7) grid (7.2,-9.2);
\draw (7.8,-7) grid (9,-9.2);
% Milieu
\draw (2,-9.8) grid (5.2,-11.2);
\draw (5.8,-9.8) grid (7.2,-11.2);
\draw (7.8,-9.8) grid (9,-11.2);
% Bas
\draw (2,-11.8) grid (5.2,-13);
\draw (5.8,-11.8) grid (7.2,-13);
\draw (7.8,-11.8) grid (9,-13);
%% Haut gauche
\foreach \j in {1,2,3}{
    \foreach \h in {1,2}{
        \draw (\j+1.5,-6.5-\h) node{\tiny$Y_{i,t_{\textcolor{blue}{\j}},\h}$};
    }
}
%% Points
\foreach \j in {1,2,3}{
    \draw (\j+1.5,-9.5) node{$\vdots$};
}
\foreach \h in {1,2}{
    \draw (5.5,-6.5-\h) node{$\cdots$};
}
%% Haut milieu
\foreach \h in {1,2}{
        \draw (6.5,-6.5-\h) node{\tiny$Y_{i,t_{\textcolor{blue}{j}},\h}$};
}
%% Points
\draw (6.5,-9.5) node{$\vdots$};
\foreach \h in {1,2}{
    \draw (7.5,-6.5-\h) node{$\cdots$};
}
%% Haut droite
\foreach \h in {1,2}{
        \draw (8.5,-6.5-\h) node{\tiny$Y_{i,t_{\textcolor{blue}{52}},\h}$};
}
%% Points
\draw (8.5,-9.5) node{$\vdots$};
%% Milieu gauche
\foreach \j in {1,2,3}{
    \draw (\j+1.5,-10.5) node{\tiny$Y_{i,t_{\textcolor{blue}{\j}},h}$};
}
%% Points
\foreach \j in {1,2,3}{
    \draw (\j+1.5,-11.5) node{$\vdots$};
}
\draw (5.5,-10.5) node{$\cdots$};
%% Milieu milieu
\draw (6.5,-10.5) node{\tiny$Y_{i,t_{\textcolor{blue}{j}},h}$};
%% Points
\draw (6.5,-11.5) node{$\vdots$};
\draw (7.5,-10.5) node{$\cdots$};
%% Milieu droite
\draw (8.5,-10.5) node{\tiny$Y_{i,t_{\textcolor{blue}{52}},h}$};
%% Points
\draw (8.5,-11.5) node{$\vdots$};
%% Bas gauche
\foreach \j in {1,2,3}{
    \draw (\j+1.5,-12.5) node{\tiny$Y_{i,t_{\textcolor{blue}{\j}},42}$};
}
%% Points
\draw (5.5,-12.5) node{$\cdots$};
%% Milieu milieu
\draw (6.5,-12.5) node{\tiny$Y_{i,t_{\textcolor{blue}{j}},42}$};
%% Points
\draw (7.5,-12.5) node{$\cdots$};
%% Milieu droite
\draw (8.5,-12.5) node{\tiny$Y_{i,t_{\textcolor{blue}{52}},42}$};
%%% Point diagonal
\draw (5.5,-9.5) node{$\ddots$};
\draw (7.5,-11.5) node{$\ddots$};
%%%%%%%%%%%%%%%
% Flèches transisitions
%%%%%%%%%%%%%%%
\draw[thick,->,>=latex] (5.5,-2) -- (5.5,-3) node[midway,right]{Notations};
\draw[thick,->,>=latex] (5.5,-5.25) -- (5.5,-6.25) node[midway,right]{Projection};

==> Tab/ARI.tex <==
0.1&0.2&1\\\midrule
 (100,50)&0.13 (0.15)&0.61 (0.15)&1 (0)\\
 (100,100)&0.32 (0.19)&0.76 (0.16)&1 (0)\\
 (1000,50)&0.33 (0.13)&0.76 (0.1)&1 (0)\\
 (1000,100)&0.55 (0.099)&0.93 (0.046)&1 (0)\\
\bottomrule

==> Tab/CE.tex <==
0.1&0.2&1\\\hline 
 (100,50)&0.76 (0.16)&0.34 (0.18)&0 (0)\\
 (100,100)&0.6 (0.17)&0.19 (0.17)&0 (0)\\
 (1000,50)&0.56 (0.15)&0.17 (0.12)&0 (0)\\
 (1000,100)&0.36 (0.14)&0.035 (0.031)&0 (0)

==> Tab/Comp_ARI.tex <==
&0.1&0.2&1\\\hline
 \multirow{2}{*}{(100,50)}&MixSeg&0.13 (0.15)&0.61 (0.15)&1 (0)\\
 &SimpleMix&0.049 (0.071)&0.22 (0.17)&0.98 (0.09)\\\hline
 \multirow{2}{*}{(100,100)}&MixSeg&0.32 (0.19)&0.76 (0.16)&1 (0)\\
 &SimpleMix&0.13 (0.11)&0.39 (0.17)&0.99 (0.076)\\\hline
 \multirow{2}{*}{(1000,50)}&MixSeg&0.33 (0.13)&0.76 (0.1)&1 (0)\\
 &SimpleMix&0.076 (0.07)&0.29 (0.14)&1 (9e-04)\\\hline
 \multirow{2}{*}{(1000,100)}&MixSeg&0.55 (0.099)&0.93 (0.046)&1 (0)\\
 &SimpleMix&0.17 (0.12)&0.41 (0.14)&1 (0)\\

==> Tab/Comp_CE.tex <==
&0.1&0.2&1\\\hline
 \multirow{2}{*}{(100,50)}&MixSeg&0.76 (0.16)&0.34 (0.18)&0 (0)\\
 &Simple&0.84 (0.1)&0.67 (0.18)&0.018 (0.089)\\\hline
 \multirow{2}{*}{(100,100)}&MixSeg&0.6 (0.17)&0.19 (0.17)&0 (0)\\
 &Simple&0.75 (0.12)&0.51 (0.18)&0.013 (0.072)\\\hline
 \multirow{2}{*}{(1000,50)}&MixSeg&0.56 (0.15)&0.17 (0.12)&0 (0)\\
 &Simple&0.82 (0.11)&0.62 (0.14)&0.00015 (0.00045)\\\hline
 \multirow{2}{*}{(1000,100)}&MixSeg&0.36 (0.14)&0.035 (0.031)&0 (0)\\
 &Simple&0.72 (0.14)&0.51 (0.16)&0 (0)\\
